Text2Mesh: Text-Driven Neural Stylization for Meshes

In this work, we develop intuitive controls for editing the style of 3D objects. Our framework, Text2Mesh, stylizes a 3D mesh by predicting color and local geometric details which conform to a target text prompt. We consider a disentangled representation of a 3D object using a fixed mesh input (content) coupled with a learned neural network, which we term neural style field network. In order to modify style, we obtain a similarity score between a text prompt (describing style) and a stylized mesh by harnessing the representational power of CLIP. Text2Mesh requires neither a pre-trained generative model nor a specialized 3D mesh dataset. It can handle low-quality meshes (non-manifold, boundaries, etc.) with arbitrary genus, and does not require UV parameterization. We demonstrate the ability of our technique to synthesize a myriad of styles over a wide variety of 3D meshes.

==> figures/ablations/000_macros.tex <==
\newif\ifdraft
\drafttrue
%\draftfalse


\newcommand{\todocolor}{\color[rgb]{1,0.5,0.0}}

\ifdraft
%Our comments:
\newcommand{\rhc}[1]{{\color{blue}[\textbf{Rana:} #1]}}
\newcommand{\sagie}[1]{{\color{red}[\textbf{Sagie:} #1]}}
\newcommand{\rl}[1]{{\color{green}[\textbf{Richard:} #1]}}
\newcommand{\roi}[1]{{\color{cyan}[\textbf{Roi:} #1]}}
\newcommand{\ojm}[1]{{\color{magenta}[\textbf{Oscar:} #1]}}
% \newcommand{\todo}[1]{{\todocolor [\textbf{CRITICAL TODO:} #1]}}

\else
\newcommand{\rhc}[1]{}
\newcommand{\sagie}[1]{}
\newcommand{\rl}[1]{}
\newcommand{\ojm}[1]{}
\newcommand{\roi}[1]{}
% \newcommand{\todo}[1]{}
\fi


\newif\ifreviewer
\reviewertrue
\reviewerfalse
\ifreviewer
\newcommand{\rev}[1]{{\color{black}#1}}
\else
\newcommand{\rev}[1]{}
\fi

% \interfootnotelinepenalty=10000 

\newcommand{\transpose}{\mathrm{T}}
\newcommand{\Vector}[1]{\left[#1\right]^\transpose}
\newcommand{\ourmethod}{Text2Mesh}
% \newcommand{\ourmethod}{MeshTexstyle}
% \newcommand{\ourmethod}{TEXTstyle}
% \newcommand{\ourmethod}{TEXTureSTYLE}

\newcommand{\clipcolor}{\color[rgb]{0.4,0.4,0.99}}
\newcommand{\contcolor}{\color[rgb]{0.2,0.95,0.7}}
\newcommand{\stylecolor}{\color[rgb]{0.9,0.4,0.4}}

%%%%%% method %%%%% 

\newcommand{\ncolor}{N_{c}}
\newcommand{\ndisplacement}{N_{d}}
\newcommand{\nshare}{N_{s}}
\newcommand{\meshstyle}{M^{S}}
\newcommand{\view}{I_{\theta}}
\newcommand{\viewfull}{I^{\text{full}}_{\theta}}
\newcommand{\viewdispl}{I^{\text{displ}}_{\theta}}
\newcommand{\meshdeform}{M_{\text{displ}}^S}
\usepackage[colorlinks,citecolor=green,urlcolor=blue,bookmarks=false,hypertexnames=true]{hyperref} 


==> figures/ablations/00_abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
% Manual authoring of 3D content is a laborious and complex process. 
In this work, we develop intuitive controls for editing the style of 3D objects. Our framework, \ourmethod{}, stylizes a 3D mesh by predicting color and local geometric details which conform to a target text prompt. We consider a disentangled representation of a 3D object using a fixed mesh input (content) coupled with a learned neural style field. In order to modify style, we obtain a similarity score between a text prompt (describing style) and a stylized mesh by harnessing the representational power of CLIP. \ourmethod{} does not require a pre-trained  generative model nor a specialized 3D mesh dataset. It can handle low-quality meshes (non-manifold, boundaries, etc.) with arbitrary genus, and does not require parameterization. We demonstrate the ability of our technique to synthesize a myriad of styles over a wide variety of 3D meshes in the wild. 
% \rl{Suggestion: mention parameterization in previous sentence instead, e.g. ``does not require pre-trained model, UV parameterization, nor specialized dataset..."}
% \sagie{Beyond text, we show that our framework can be used to stylize input meshes using a target image, a target mesh or even multiple targets.}
% - we do this by defining the process as style transfer
% - we stylize any 3D mesh in the wild , by coloring and local geometric displacements using the power of CLIP. and don't require UV parameterization.
% - A notable advantange of our technique is the ability to handle poor-quality meshes.
% - Our framework is general. We do not require a specialized 3D datatset, and demonstrate the ability to handle a variety of content and styles.
% - 
%   Manipulating 3D meshes by hand is a time-consuming and laborious process. Motivated by the success of CLIP-guided generative models, we propose a method to automatically color and deform a mesh to match the style of a given text prompt, image, or text-image combination using a stylization network and an off-the-shelf differentiable renderer. Unlike previous methods, our method does not require a pre-trained generative model to guide search in CLIP space, and thus our results are agnostic to any particular dataset. Instead, we find that the combination of an expressive fourier-feature stylization network, the 3D geometric prior imposed by meshes and careful augmentation training are enough to produce realistic results.
%\\
%\\%2 line spaces are required after the abstract
\end{abstract}

==> figures/ablations/01_intro.tex <==
\begin{figure*}
    \centering
    \newcommand{\pl}{0.5}
    \newcommand{\upl}{10}
    \newcommand{\ml}{1.5}
    \newcommand{\uml}{16}
    \newcommand{\urp}{14.5}
    \begin{overpic}[width=0.97\textwidth]{figures/shoe_long_v2.jpg}
    \put(16,  \pl){\textcolor{black}{Cactus}}
    \put(34,  \pl){\textcolor{black}{Bark}}
    \put(50,  \pl){\textcolor{black}{Brick}}
    \put(60,  \pl){\textcolor{black}{Wood}}
    \put(58,  \upl){\textcolor{black}{Stained Glass}}
    \put(73,  \pl){\textcolor{black}{Chainmail}}
    \put(75,  \upl){\textcolor{black}{Fur}}
    \put(88,  \pl){\textcolor{black}{Wicker}}
    \put(85,  \upl){\textcolor{black}{Burgundy Crochet}}
    % \put(93,  \pl){\textcolor{black}{brick}}
    % \linethickness{1pt}
    % \put(0,0.5){\color{black}\vector(1,0){100}}
    % \vspace{2pt}
    \end{overpic}
    \begin{overpic}[width=0.97\textwidth]{figures/vase_long_v2.jpg}
    \put(10,  \ml){\textcolor{black}{Colorful Crochet}}
    \put(27,  \ml){\textcolor{black}{Colorful Doily}}
    \put(47,  \ml){\textcolor{black}{Cactus}}
    \put(58,  \ml){\textcolor{black}{Embroidered}}
    \put(60,  \uml){\textcolor{black}{Wood}}
    \put(74,  \ml){\textcolor{black}{Beaded}}
    \put(74,  \uml){\textcolor{black}{Wicker}}
    \put(87,  \ml){\textcolor{black}{Chainmail}}
    \put(89,  \uml){\textcolor{black}{Bark}}
    \end{overpic}
    \begin{overpic}[width=0.97\textwidth]{figures/horse_long.jpg}
    \put(14,  \pl){\textcolor{black}{Robot}}
    \put(28,  \pl){\textcolor{black}{Poncho}}
    \put(43,  \pl){\textcolor{black}{Metal Scales}}
    \put(60,  \pl){\textcolor{black}{Wood}}
    \put(60,  \urp){\textcolor{black}{Cactus}}
    \put(74,  \pl){\textcolor{black}{Beaded}}
    \put(72,  \urp){\textcolor{black}{Spotted Fur}}
    \put(86,  \pl){\textcolor{black}{Embroidered}}
    \put(88,  \urp){\textcolor{black}{Wicker}}
    \end{overpic}
    % \\\vspace{3mm}
    % \begin{overpic}[width=\textwidth]{figures/alien_long.jpg}
    % \put(15,  \pl){\textcolor{black}{Cactus}}
    % \put(34,  \pl){\textcolor{black}{Bark}}
    % \put(50,  \pl){\textcolor{black}{Brick}}
    % \put(62,  \pl){\textcolor{black}{Wood}}
    % \put(72,  \pl){\textcolor{black}{Chainmail}}
    % \put(80,  \pl){\textcolor{black}{burgonedy crochet}}
    % \put(93,  \pl){\textcolor{black}{brick}}
    % \end{overpic}
    \caption{Given a source mesh (gray), our method produces stylized meshes (containing color and local geometric displacements) which conform to various target texts. Insets show a close up of the stylization (with color), as well as the underlying geometry produced by the deformation component (without color). Insets of the source mesh are also shown on the left most column. } % \rhc{TODO someone reread this, its good!}}  % \rhc{TODO: finish captioning}\roi{Trojan Horse!!} } 
\label{fig:gallery}
\vspace{-0.5cm}
\end{figure*}
% \rl{\textbf{Shoes:} burgundy crochet, bark, wood, fur, chainmail, cactus, wicker, stained glass, brick. \textbf{Vase: } colorful crochet, bark, wood, colorful doily, chainmail, cactus, wicker, beaded, embroidered. \textbf{Horse: } poncho, bark, robot, spotted fur, metal scales, cactus, wicker, beaded, embroidered. \textbf{Alien: } space alien, wood, robot, happy, metal scales, cactus, wicker, brick, embroidered}
\vspace{-25pt}
\section{Introduction}
\label{sec:intro}
\vspace{-5pt}
Editing visual data to conform to a desired style, while preserving the underlying content, is a longstanding objective in computer graphics and vision~\cite{Hertzmann2000, gatys2016image, adain, isola2017image, kolkin2019style}. Key challenges include proper formulation of content, style, and the constituents for representing and modifying them.

%%% highest level goal summary %%%%
To edit the style of a 3D object, we adapt a formulation of geometric content and stylistic appearance commonly used in computer graphics pipelines~\cite{renderingbook}. We consider \emph{content} as the global structure prescribed by a 3D mesh, which defines the overall shape surface and topology. 
We consider \emph{style} as the object's particular appearance or affect, as determined by its color and fine-grained (local) geometric details. We propose expressing the desired style through natural language (a text prompt), similar to how a commissioned artist is provided a verbal or textual description of the desired work. This is facilitated by recent developments in joint embeddings of text and images, such as  CLIP~\cite{clip}.

% \rl{I feel like as an outside reader I would be confused about what it actually means to modify the mesh content given the somewhat loose definition given. Can we say explicitly what kind of transformations we \textbf{dont} allow for? e.g. pose changes, changes to shape category, etc. }
%%% highest level method summary %%%%
A natural cue for modifying the appearance of 3D shapes is through 2D projections, as they correspond with how humans and machines perceive 3D geometry. 
%A neural stylization network is used synthesize color and local geometric details over the input shape, \textit{without} modifying the given 3D mesh content.
%Our system uses a neural optimization that is guided by multiple 2D (CLIP-embedded) views of a 3D stylized mesh. 
% The weights of a neural network are optimized for a given 3D mesh to adhere to the desired style described in the text. 
We use a neural stylization network to synthesize color and local geometric details over the 3D input shape, \textit{without} modifying the given mesh content. The weights of our network are optimized such that the resulting 3D stylized mesh adheres to the style described by text. In particular, our neural optimization is guided by multiple 2D (CLIP-encoded) views of the stylized mesh matching our target text. 
Results of our technique, called \ourmethod{}, are shown in \cref{fig:teaser}.
Our method produces different colors and local deformations for the same 3D mesh content to match the specified text. Moreover, \ourmethod{} produces structured textures that are aligned with salient features (\eg bricks in \cref{fig:gallery}), without needing to estimate sharp 3D curves or a mesh parameterization~\cite{Li:2018:OptCuts, sharp2018variational}.
Our method also demonstrates global understanding; \eg in \cref{fig:humans} human body parts are stylized in accordance with their semantic role.
% our method demonstrates a global semantic understanding of humans. Different body parts such legs, head and muscles are stylized appropriately in accordance with their semantic role, and these styles are blended seamlessly across the surface to form a cohesive stylization. 

\begin{figure*}
    \centering
    \newcommand{\pl}{-1}
    \begin{overpic}[width=\textwidth]{figures/humans.jpg}
    % \put(40,  20){\textcolor{black}{\textbf{Text Style}}}
    \put(2,  \pl){\textcolor{black}{Input}}
    \put(10.5,  \pl){\textcolor{black}{Steve Jobs}}
    \put(23,  \pl){\textcolor{black}{Yeti}}
    \put(30,  \pl){\textcolor{black}{Astronaut}}
    \put(39,  \pl){\textcolor{black}{Buzz Lightyear}}
    \put(53,  \pl){\textcolor{black}{Ninja}}
    \put(62,  \pl){\textcolor{black}{Lawyer}}
    \put(73,  \pl){\textcolor{black}{Messi}}
    \put(82,  \pl){\textcolor{black}{Batman}}
    \put(92,  \pl){\textcolor{black}{Hulk}}
    \end{overpic}
    \caption{Given the same input bare mesh, our neural style field produces deformations for outerwear of various types (capturing fine details such as creases in clothing and complementary accessories), as well as distinct features such as muscle and hair. 
    The synthesized colors consider both local geometric details and global part-aware semantics. 
    Insets of the source mesh are shown in the top row and insets of the stylized output are shown in the middle (uncolored) and bottom (colored) rows.}
\label{fig:humans}
\vspace{-0.5cm}
\end{figure*}
% Our method produces different styles (color and local geometry) over the same input 3D mesh. 
%%%% representations: CONTENT / STYLE , EXPLICIT / IMPLICIT %%%%%
We use the weights of a neural network to encode a style field over the \emph{explicit} mesh surface. Meshes faithfully portray 3D shapes and can accurately represent sharp, extrinsic features using a high level of detail.
Our neural style field is \textit{complementary} to the mesh content, and appends colors and small displacements to the input mesh. Specifically, our neural style field maps points on the mesh surface to style attributes (\ie, RGB colors and displacements).

%%%% how we use CLIP %%%%%
We guide the neural style field by rendering the stylized 3D mesh from multiple 2D views and measuring the similarity of those views against the target text, using CLIP's space.
% CLIP provides a valuable similarity score between (meaningful) text-image pairs. 
However, a straightforward optimization of the 3D stylized mesh which maximizes the CLIP similarity score converges to a degenerate (\ie noisy) solution (see \cref{fig:ablations}) \roi{this phenomenon is described by Fort in \cite{Fort2021CLIPadversarial,Fort2021CLIPadversarialstickers}}.
% Yet, employing CLIP directly for synthesis is non-trivial and naively tends towards degenerate solutions.
Specifically, we observe that the joint text-image embedding space contains an abundance of \textit{false positives}, where a valid target text and a degenerate image (\ie noise, artifacts) result in a high similarity score. 
Therefore, employing CLIP for stylization requires careful regularization.

%%%% PRIORS %%%%%
To this end, we leverage multiple \emph{priors} to effectively guide our neural stylization field. The 3D mesh input acts as a \emph{geometric prior} that imposes global shape structure, as well as local details that indicate the appropriate position for stylization. The weights of the neural stylization network act as a \emph{neural prior} (\ie regularization technique), which tends to favor smooth solutions~\cite{SpectralBias, hanocka2020point2mesh, ulyanov2018deep}. In order to produce accurate styles which contain high-frequency content with high fidelity, we use a frequency-based positional encoding~\cite{FourierFeaturesNetwork}.
We garner a strong signal about the quality of the neural style field by rendering the stylized mesh from multiple 2D views and then applying 2D augmentations. This results in a system which can effectively avoid degenerate solutions, while still maintaining high-fidelity results.

%%% focus on text,  but also other things %%%%
The focus of our work is text-driven stylization, since text is easily modifiable and can effectively express complex concepts related to style. Text prescribes an abstract notion of style, allowing the network to produce different valid stylizations which still adhere to the text. Beyond text, our framework is general and easily extends to additional target modalities, such as images and even 3D meshes. 

%%%% what we show %%%%%
In summary, we present a technique for the semantic manipulation of style for 3D meshes, harnessing the representational power of CLIP. 
Our system combines the advantages of \emph{explicit} mesh surfaces and the generality of neural fields to facilitate intuitive control for stylizing 3D shapes. A notable advantage of our framework is its ability to handle low-quality meshes (\eg, non-manifold) with arbitrary genus. We show that \ourmethod{} can stylize a variety of 3D shapes with many different target styles.


==> figures/ablations/02_related.tex <==
\section{Related Work}
\label{sec:rw}
% The results here uses a symmetric prior assumption, by reflecting the input coordinates $\Phi\left(x,y,z\right)=\left(x,y,\left|z\right|\right)$ as discussed in \roi{xx}.
% \sagie{I think the section is now too long - need to cut it down}
% \rhc{TODO: add a line and cite works which do 3D shape analysis for texturing~\cite{xu2009feature}, could also go in intro.}
% \rhc{maybe we do not need this intro paragraph. I think it will be clear after reading the RW that nobody can do what we do} \sagie{ok, changed this now}
% While, we introduce a novel setting of text-driven manipulation of style for 3D meshes, individual components of our method are related to 
% % While the setting of neural style transfer has been widely investigated in the context of images and videos, as far as we can ascertain, our setting of text-driven manipulation of style for 3D meshes is novel. We consider the relevant literature of 
% \emph{text-driven manipulations}, \emph{style transfer} and to \emph{neural editing} methods. We therefore consider the relavent literature here. 
% \sagie{change according to what is actually done}

% \vspace{0.1cm}
\noindent\textbf{Text-Driven Manipulation.}\quad 
% \textbf{}
% \sagie{text to image, scene graph to image, other}
% Much of the literature considers the task of text-to-image generation~\cite{reed2016generative, xu2018attngan, zhang2017stackgan, zhang2018stackgan++, li2019object, koh2021text}. %\rhc{not sure about these?}.
% [10, 31, 27] [22]



\roi{Our work is influenced by the recent burst on optimizing visual representations supervised by a pre-trained CLIP~\cite{clip} model. 
CLIP learns a vision-language embedding space, thus, it allows to quantify the similarity of (image, text) pairs and to optimize different representations to minimize this distance.
StyleCLIP~\cite{patashnik2021styleclip} and VQGAN-CLIP~\cite{vqganclipnotebook, esser2020taming, unpublished2021clip} uses the latent spaces of pre-trained GANs to manipulate generated images. Introducing a pre-trained GAN in their pipeline limits the models to results producible by the given generators. Thus, doesn't fully utilize the capabilities of CLIP and its variety of visual concepts.
Concurrent to us, \cite{chefer2021image} uses a GAN for image stylization.


Concurrent work of \cite{stylegannada} uses CLIP for zero-shot domain adaptation of  StyleGAN~\cite{karras2019style,  karras2020analyzing} generators. This allows to use some controls from the original GAN in the resulted GAN. However, it is limited to adapt to domains that are close to the original domain, thus only slightly mitigates the need of a large dataset, and heavy compute times when a new domain is required. StyleGAN has its on limitations when it comes to image manipulations: it requires a non intuitive search for existing editing directions and a very limited set of such directions exists, compared to the amount of editing command one can verbally express. 

Concurrent works to ours tries to extend CLIP driven optimizations to 3D. 
Unconditional 3D shape generation using 3D voxels (\cite{clipforge}) and human body model from SMPL~\cite{smpl} (\cite{clipmatrix}) this work is coupled with a specific given source content. All of the above requires data-driven prior, given by a training data-set or a pre-trained model, ontop of the CLIP supervision.


Similar to our method, Frans \etal~\cite{clipdraw} generates text-guided vector graphics without a pre-trained generator. It is used to generate simple drawings. however, unlike our method, CLIPDraw is built for 2D outputs. and  doesn't utilize a neural field nor stylizing a given content input. a followup work \cite{styleclipdraw} uses similar technique to convey style, but introduces a pre-trained CNN with real data biases. 
}
Our work is similar in spirit to image manipulation techniques controlled through textual descriptions encoded by CLIP~\cite{clip}. 
% (Contrastive Language-Image Pre-training)
CLIP learns to project images and text into a multi-modal embedding space.
%by training over a large number of pairs of images and text collected from the internet.
StyleCLIP~\cite{patashnik2021styleclip} uses the latent space of a pre-trained StyleGAN~\cite{karras2019style,  karras2020analyzing} to manipulate human faces guided by the CLIP.  embedding of text prompts. 
% Subsequent approaches generate a variety of text-driven content beyond human faces~
VQGAN-CLIP~\cite{vqganclipnotebook, esser2020taming, unpublished2021clip} extends StyleCLIP to a variety of text-driven content. 
% beyond human faces
% using a pre-trained model of VQ-GAN
% ~\cite{esser2020taming, unpublished2021clip}. 
Concurrent work of \cite{stylegannada} and \cite{chefer2021image} use StyleGAN and CLIP simultaneously for domain adaptation and 2D image stylization, respectively. 
% TargetCLIP~\cite{chefer2021image} and  use the CLIP embedding in order to adapt StyleGAN generators to new domains, and TargetCLIP~\cite{chefer2021image} which use additivity in the both the SyleGAN and CLIP space to achieve higher level abstractions then textures and colors for style transfer. 
CLIP has been used for unconditional 3D shape generation using 3D voxels~\cite{clipforge}.
% \cite{clipforge} use CLIP for unconditional 3D shape generation using 3D voxels. %, and trains over a 3D shape dataset. 
Unlike our method which only uses CLIP for semantic association, these approaches leverage the data-driven prior of a pre-trained generative model (such as StyleGAN) or a 3D shape dataset to % effectively explore the natural image manifold, which helps 
prevent degenerate solutions. They are also used to convey content and not style. 
CLIPDraw~\cite{clipdraw} generates text-guided vector graphics without a pre-trained generator. Similar to our method, it is used to convey style \roi{they don't covey style style, they generate drawings can mention StyleClipDraw \cite{styleclipdraw} as a concurrent work that convey style in 2D} without needing to rely on a specialized dataset; however, unlike our method, CLIPDraw is built for 2D outputs. \roi{and  doesn't utilize a neural field nor stylizing a given content input}

% CLIPDraw~\cite{clipdraw} generates text-guided 2D vector graphics without a pre-trained generator, and similar to our method, is used to convey style and does not rely on a specialized dataset. 
% While prior CLIP-based synthesis approaches focused on generating \textit{content}, CLIPDraw and our method use CLIP for conveying \textit{style}.
% \rhc{\underline{SAGIE, approve this:}}
% Recent work uses CLIP for unconditional 3D shape generation using a 3D voxels, and trains over a 3D shape dataset~\cite{clipforge}. Different from our work, they generate 3D content without style (neither color nor local geometry).
A concurrent work uses CLIP to optimize the parameters of the SMPL~\cite{smpl} human body model~\cite{clipmatrix}. 
% , such as the shape parameters and texture colors from a UV-map to create digital creatures~\cite{clipmatrix}. 
In contrast, our framework is not tied to a particular 3D object structure, and can generate global part-aware semantics without any explicit priors or supervision.
% (\eg see \cref{fig:humans}). I am not mentionehing this as this might need comparision.  
Prior to CLIP, text-driven control for deforming 3D shapes was explored~\cite{yumer2015semantic, yumer2016learning} using specialized 3D datasets. 

% \rhc{
% Other methods of style control such as StyleGAN~\cite{Stylegan-Ada} involve the complicated and unintuitive procedure of identifying a desired direction in the latent space. Our method is not limited to these pre-defined directions and allows for the expression of a much broader range of styles, including ones potentially out-of-distribution.
% }
\vspace{0.1cm}
\noindent\textbf{Geometric Style Transfer in 3D.}\quad 
Some approaches analyze 3D shapes and identify similarly shaped geometric elements and parts which differ in style~\cite{xu2010style, li2013curve, lun2015elements, hu2017co, yu2018semi}.
%
Others transfer geometric style based on content/style separation~\cite{yin2019logan, cao2020psnet, segu20203dsnet}.
% \rhc{SAGIE: check this... I extended discussion as these are pretty related. might be good to even add more about why they are unrelated.} \sagie{great!}
3DStyleNet~\cite{yin20213dstylenet} edits shape content using a part-aware deformation and texture map. % guided by a target mesh.
Mesh Renderer~\cite{kato2018neural} changes color and geometry driven by a target image.
\cite{liu2018paparazzi} stylize a 3D shape by adding geometric detail (without color), and ALIGNet~\cite{hanocka2018alignet} deforms a template shape to a target one.
Other approaches are specific to categories of furniture~\cite{lun2016functionality}, 3D collages~\cite{gal20073d}, LEGO~\cite{lennon2021image2lego}, and portraits~\cite{han2021exemplar}.
% 3DStyleNet~\cite{yin20213dstylenet} recently proposed a technique for editing both the shape (content) and texture of a source mesh towards target mesh. Mesh Renderer~\cite{kato2018neural} stylizes 3D shape from a 2D target image by changing color and geometry. \cite{liu2018paparazzi} stylize a 3D shape by adding geometric detail (no color), and ALIGNet~\cite{hanocka2018alignet} deforms a template shape to a target one.
% Since 3DStyleNet predicts a smooth deformation (using linear blend skinning) for each semantic part in the object to modify the mesh content. Such low-frequency deformations are suited for changing the overall shape, semantic structure, and even pose of an object, while still preserving fine-grained geometric details~\cite{neuralcages}.
These methods rely on 3D datasets. 
Some techniques do not rely on a dataset, such as for
%that capture a variety of different styles. 
% Some techniques do not rely on an externally defined dataset for %s have also been explored. 
synthesizing geometric textures~\cite{hertz2020deep} or mesh refinements~\cite{liu2020neural}, using a single mesh exemplar as a target. Shapes can be edited to contain cubic stylization~\cite{liu2019cubic}, or stripe patterns~\cite{knoppel2015stripe}. Unlike these methods, we consider a wide range of stylizations, guided by an intuitive and compact specification of style. 
% Our method modifies both the color and local geometry of a source mesh through a target text which is a rather intuitive and compact specification of style. 

% \textbf{Texture Transfer in 3D.} 
\vspace{0.1cm}
\noindent\textbf{Texture Transfer in 3D.}\quad 
Aspects of a 3D mesh style can be controlled by 
% A common technique for controlling the style of meshes is by 
texturing a surface through mesh parameterization~\cite{sorkine2002bounded, sharp2018variational, Li:2018:OptCuts, gillespie2021discrete}. 
%Mesh parameterization aims to map the 3D surface into a 2D plane (or to another surface) with low-distortion, which is a fundamental problem in computer graphics that remains challenging. 
However, most parameterization approaches place strict requirements on the quality of the input mesh (e.g., a manifold, non-intersecting, and low/zero genus), which do not hold 
% Yet, this assumption does not hold 
for most meshes in the wild~\cite{sharp2021int}. We avoid parameterization altogether and opt to manipulate appearance using a neural field which provides a style value (\ie, an RGB value, or a displacement) for every vertex on the mesh. 
% \rl{Maybe also say here that the point of the neural field is to learn style in a way that is agnostic to particular discretization of the surface?} \rhc{not here.. we get there in the method.}
While recent work explored a neural representation of texture~\cite{oechsle2019texture}, we consider both color and local geometry changes for the manipulation of style.  
% \rhc{TODO \cite{oechsle2019texture}} \sagie{should we move this completely to implicit section? add here texture fields}


% \textbf{Neural Priors and Neural Field Representations.} 
\vspace{0.1cm}
\noindent\textbf{Neural Priors and Neural Field Representations.}\quad 
A recent line of work leverages 
% the inductive bias of neural networks (mostly avoid the need for large datasets) to accomplish
the inductive bias of neural networks for 
tasks such as image denoising~\cite{ulyanov2018deep}, surface reconstruction~\cite{hanocka2020point2mesh}, point cloud consolidation~\cite{metzer2021self}, image synthesis, and editing~\cite{ingan, shaham2019singan, zhao2018deepsim}. 
Our framework leverages the inductive bias of neural networks to act as a prior which guides \ourmethod{} away from degenerate solutions present in the CLIP embedding space.
Specifically, our stylization network acts as a neural prior, which leverages positional encoding~\cite{FourierFeaturesNetwork} to synthesize fine-grained stylization details.
% One such important neural prior is introduced by our stylization network, which is a specific realization of a neural coordinate field network (similar to \cite{FourierFeaturesNetwork}).

% As CLIP's space contains sharp discontinuities and our target prompt only partially specifies the desired source style, our method incorporates a number of priors which encourage smooth and desirable results, as described in \cref{sec:intro,sec:method}.  
% In the context of 3D object modeling, 
% \roi{NeRF~\cite{mildenhall2020nerf} and its following works \cite{zhang2020nerf++, park2020deformable,yu2021pixelnerf}}
NeRF~\cite{mildenhall2020nerf} and follow ups~\cite{zhang2020nerf++, park2020deformable,yu2021pixelnerf} have demonstrated success on 3D scene modeling.
% using 2D image views. 
They leverage a neural field to represent 3D objects using network weights.
However, neural fields commonly \emph{entangle} geometry and appearance, which limits separable control of content and style.
Moreover, they struggle to accurately portray sharp features, are slow to render, and are difficult to edit.  Thus, several techniques were proposed enabling ease of control~\cite{gpwithneuralfields}, and introducing acceleration strategies~\cite{reiser2021kilonerf}. % \rhc{TODO addd other citations} 
Our method uses a disentangled representation of a 3D object using an \emph{explicit} mesh representation of shape and an \emph{implicit} neural style field which controls appearance. 
Such formulation avoids parametrization, and can be used to easily manipulate appearance and generate high resolution outputs. 
% Our formulation enjoys a disentangled representation of shape and appearance on the one hand, and the ability to avoid parameterization, easily manipulate appearance, and generate high resolution outputs on the other.




==> figures/ablations/03_overview.tex <==
% \section{Overview}

% Our approach learns to generate neural style over a 3D mesh content using positional encoding network~\cite{FourierFeaturesNetwork}. The network is driven by a target image or text, which is passed through a pre-trained CLIP model to obtain the desired style embedding $S \in \mathbb{R}^{512}$.

% We train a network to learn to map a point $x \in \mathbb{R}^3$ on the mesh surface to a style attribute (\eg, an RGB color or a displacement). The stylized mesh is passed to a differential renderer~\cite{chen2019learning}, which is used to render multiple views of the neural style mesh. Each image is passed to a pre-trained CLIP model to obtained a predicted style embedding $\hat{S} \in \mathbb{R}^{512}$. The difference in the desired and predicted style embedding is used as a signal to update the weights of the neural style network. 

% \rhc{this is unfinished. here's some remaining todos:
% - discuss how we render colors between triangles by inserting a "fake" vertex, which gives us the ability to learn this mapping at a resolution which is sort of invariant to the triangulation (show it in the experiments...)

% - discuss some of the augmentations needed to avoid the adversarial solution (right now I believe we only use 2D perspective, but that might change, so keep it general I guess)

% - talk about displacements along the normal, which are smooth by construction, and sort of independent from the mesh content

% - talk a bit about the architecture, although this might change. currently we use FFN.

% - The loss is cosine similarity
% }

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{example-image-a}
%     \caption{\rhc{Overview Figure.}}
%     \label{fig:overview}
% \end{figure*}

==> figures/ablations/04_method.tex <==
\begin{figure}[t!]
    \centering
    \newcommand{\inpcolor}{\color[rgb]{0.4,0.96,0.4}}
    \newcommand{\fieldcolor}{\color[rgb]{0.9,0.8,0.5}}
    \newcommand{\augcolor}{\color[rgb]{0.5,0.5,0.9}}
    \newcommand{\semcolor}{\color[rgb]{0.9,0.4,0.4}}
    \includegraphics[width=\columnwidth]{figures/pipeline.pdf}
    \caption{\ourmethod{} modifies an {\inpcolor \textbf{input mesh}} to conform to the {\inpcolor \textbf{target text}} by predicting color and geometric details. The weights of the {\fieldcolor \textbf{neural style network}} are optimized by {\augcolor \textbf{rendering}} multiple 2D images and applying {\augcolor \textbf{2D augmentations}}, which are given a similarity score to the target from the CLIP-based {\semcolor \textbf{semantic loss}}.}
    \label{fig:overview}
    \vspace{-0.3cm}
\end{figure}

\vspace{-1pt}
\section{Method}
\label{sec:method}
An illustration of our method is provided in \cref{fig:overview}. 
As an overview, the 3D object \emph{content} is defined by an input mesh $M$ with vertices $V \in \mathbb{R}^{n \times 3}$ and faces $F \in \{1, \hdots, n\}^{m \times 3}$, and is fixed throughout training. The object's \emph{style} (color and local geometry) is modified to conform to a target text prompt $t$, resulting in a stylized mesh $\meshstyle$. The neural field learns to map points on the mesh surface $p \in V$ to an RGB color and displacement along the normal direction. We render $\meshstyle$ from multiple views and apply 2D augmentations that are encoded using CLIP. The CLIP similarity between the rendered and augmented images and the target text is used as a signal to update the neural network weights. 

\subsection{Neural Style Field Network}
Our network produces a style attribute for every vertex which results in a \textit{style field} defined over the entire shape surface.
Our style field is represented as an MLP, which maps a point $p \in V$ on the mesh surface $M$ to a color and displacement along the surface normal $\left(c_p,d_p\right) \in (\mathbb{R}^3, \mathbb{R}$). This formulation tightly couples the style field to the source mesh, enabling only slight geometric modifications. 
% \rl{maybe add a short phrase to this sentence to indicate what we actually mean by style field?}

In practice, we treat the given vertices of $M$ as query points into this field, and use a differentiable renderer to visualize the style over the given triangulation. Increasing the number of triangles in $M$ for the purposes of learning a neural field with finer granularity is trivial, \eg, by inserting a degree $3$ vertex (see Supplementary). Even using a standard GPU (11GB of VRAM) our method handles meshes with up to $180$K triangles. We are able to render stylized objects using very high resolutions, as shown in the Supplementary.
\begin{figure}[h]
    \centering
    \newcommand{\pl}{-3}
    \newcommand{\vl}{-8}
    \begin{overpic}[width=\columnwidth]{figures/ablations/ablations_v2.jpg}
    % \put(33,  50){\textcolor{black}{\textit{Candle made of bark}}}
    \put(14,  \pl){\textcolor{black}{\textit{full}}}
    \put(23, \pl){\textcolor{black}{\textit{$-$net}}}
    \put(35, \pl){\textcolor{black}{\textit{$-$aug}}}
    \put(46,  \pl){\textcolor{black}{\textit{$-$FFN}}}
    \put(58,  \pl){\textcolor{black}{\textit{$-$crop}}}
    \put(69,  \pl){\textcolor{black}{\textit{$-$displ}}}
    \put(83,  \pl){\textcolor{black}{\textit{$-$3D}}}
    \put(14,  \vl){\clipcolor{$\textbf{0.36}$}}
    \put(24,  \vl){\clipcolor{$0.26$}} %net
    \put(36,  \vl){\clipcolor{$0.20$}} %aug
    \put(48,  \vl){\clipcolor{$0.26$}} %FFN
    \put(60,  \vl){\clipcolor{$0.30$}} %crop
    \put(71,  \vl){\clipcolor{$0.29$}} %geoloss
    \put(84,  \vl){\clipcolor{$0.29$}} %-3D
    \end{overpic} 
    % \vspace{-8pt}
    \vspace{2pt}
    % \newcommand{\wo}{w/o}
    % \newcommand{\wo}{without}
    \caption{Ablation on the priors used in our method (\emph{full}) for a candle mesh and target of `Candle made of bark': w/o our style field network (\textit{$-$net}), w/o 2D augmentations (\textit{$-$aug}), w/o positional encoding (\textit{$-$FFN}), w/o crop augmentations for $\Psi_{\text{displ}}$ (\textit{$-$crop}), w/o the \textit{geometry-only} component of $L_{\text{sim}}$ (\textit{$-$displ}), and learning over a 2D plane in 3D space (\textit{$-$3D}). We show the {\clipcolor{CLIP score}} ($\text{sim}(\hat{S}^{\text{full}}, \phi_{\text{target}})$); see Sec.~\ref{sec:method} for more details.
    }
    \label{fig:ablations}
    \vspace{-0.3cm}
\end{figure}

Since our neural style field uses low-dimensional coordinates as input to an MLP, this exhibits a spectral bias~\cite{SpectralBias} toward smooth solutions (\eg see~\cref{fig:ablations}). To synthesize high-frequency details, we apply a positional encoding using Fourier feature mappings, which enables MLPs to overcome the spectral bias and learn to interpolate high-frequency functions~\cite{FourierFeaturesNetwork}. For every point $p$ its positional encoding $\gamma(p)$ is given by:
% . We then apply positional encoding $\gamma$ on $p$:
% The point $p$ goes through a positional encoding using $\gamma$ \begin{equation}
\begin{align}
\gamma\left(p\right) = \left[\cos\left(2 \pi \mathbf Bp\right), \sin\left(2 \pi \mathbf Bp\right)\right]^\transpose
\label{eq:positional}
\end{align}
where $\mathbf{B} \in \mathbb{R}^{n \times 3}$ is a random Gaussian matrix where each entry is randomly drawn from $\mathcal{N}\left(0,\sigma^2\right)$. The value of $\sigma$ is chosen as a hyperparameter which controls the frequency of the learned style function. We show in \cref{sec:control} that this allows for user control over the frequency of the output style. 
% level of frequency details produced for the synthesized output, as shown in \cref{sec:frequency}. \sagie{Together with the ability to control the density of vertices in the mesh, this allows for a fine-grained control of output geometry.}
% This enables some user control over the frequency of the synthesized style. 

First, we normalize the coordinates $p \in V$ to lie inside a unit bounding box.
Then, the per-vertex positional encoding features $\gamma(p)$ are passed as input to an MLP $\nshare$, which then branches out to MLPs $N_d$ and $N_c$. % which predicts color. 
% By controlling the standard deviation of $B$, we show that the Fourier feature encoding has the added benefit of enabling some user control over the frequency of the synthesized style (see \cref{fig:frequency}).
Specifically, the output of $N_c$ is a color $c_p\in[0,1]^{3}$, and the output of $N_d$ is a displacement along the vertex normal $d_p$. To prevent content-altering displacements, we constrain $d_p$ to be in the range $(-0.1, 0.1)$. To obtain our stylized mesh prediction $\meshstyle$, every point $p$ is displaced by $d_p \cdot \vec{n}_p$ and colored by $c_p$. Vertex colors propagate over the entire mesh surface using an interpolation-based differentiable renderer~\cite{dibr}. 
During training we also consider the displacement-only mesh $M^S_{\text{displ}}$, which is the same as $\meshstyle$ without the predicted vertex colors (replaced by gray). Without the use of $M^S_{\text{displ}}$ in our final loss formulation (\cref{eq:fullloss}), the learned geometric style is noisier ($-displ$ ablation in \cref{fig:ablations}). 
% The use of $M^S_{text{displ}}$ enforces the network to produce purely geometric refinements, regardless of color. 
% % which we observe to be more difficult to optimize compared with color.
% We show in the $-displ$ ablation in \cref{fig:ablations} that without this additional encouragement, the learned geometric style is noisier. \sagie{the definition of $M^S_{text{displ}}$ doesnt enforce anything, it is the loss!!! which we talk about later.}

% where every point $p$ is displaced by $d_p \cdot \vec{n}_p$, but not colored by $c_p$. Instead, we color the mesh grey and use $M^S_{text{displ}}$ to give geometry-only loss \ojm{fix this sentence eventually}.   
% This encourages the network to emphasize displacing the geometry during training, which tends to be optimized more slowly than the color. \rhc{explain why, what's the intuition here? } \sagie{this is unclear, we wish to say the lr for geometry network is lower?}
% \sagie{defint this here for displacement only and for color and displacement and then use it below} 
% \sagie{make sure to add rendering time in the training details, and refer to this section in the supplementary}

% \sagie{talk about displacements along the normal, which are smooth by construction, and sort of independent from the mesh content}

% \sagie{describe architecture of FFN here now, positional encoding network~\cite{FourierFeaturesNetwork}}
% \vspace{-10pt}
\subsection{Text-based correspondence} 
% \vspace{-10pt}
Our neural optimization is guided by the multi-modal embedding space provided by a pre-trained CLIP~\cite{clip} model. 
Given the stylized mesh $\meshstyle$ and the displaced mesh $\meshdeform$, we sample $n_{\theta}$ views around a pre-defined anchor view and render them using a differentiable renderer. For each view, $\theta$, we render two 2D projections of the surface, $\viewfull$ for  $M^S$ and $\viewdispl$ for $\meshdeform$. Next, we draw a 2D augmentation $\psi_{\text{full}} \in \Psi_{\text{full}}$ and $\psi_{\text{displ}} \in \Psi_{\text{displ}}$, for $\viewfull$ and $\viewdispl$, respectively (details in \cref{sec:viewpoint}). We apply the augmentations to each view, and then encode it into CLIP space. Finally, we average the embeddings across all views: 
% Next, we apply a set of 2D augmentations for $\viewfull$ and $\viewdispl$. Let $\Psi_{text{full}}$ and $\Psi_{text{displ}}$ be a set of $n_{text{aug}}$ augmentations drawn at random as described below. We apply each of the augmentations in $\Psi_{text{full}}$ and $\Psi_{text{displ}}$ on $\viewfull$ and $\viewdispl$ respectively. We encode each augmented view into CLIP space and average the embeddings across all views:
\begin{align}
\hat{S}^{\text{full}} &= \frac{1}{n_\theta} \sum_{\theta} E\left(\psi_{\text{full}}\left(\viewfull\right)\right) \in \mathbb{R}^{512} \\ 
% \end{align}
% \begin{align}
\hat{S}^{\text{displ}} &= \frac{1}{n_\theta} \sum_{\theta} E\left(\psi_{\text{displ}}\left(\viewdispl\right)\right) \in \mathbb{R}^{512}.
% \hat{S}^{\text{displ}}_{\theta_2} &= \frac{1}{n_{text{aug}}}E(\psi^i_2(\viewdispl)) \in \mathbb{R}^{512}
\end{align}
% That is, we consider an augmented representation of our input mesh as the average of its embedding from multiple augmented views.
That is, we consider an augmented representation of our input mesh as the average of its embedding from multiple augmented views.
We also apply the $\psi_{\text{displ}}$ augmentation to $\viewfull$ for a third augmented embedding. \begin{align}
\hat{S}^{\text{local}} &= \frac{1}{n_\theta} \sum_{\theta} E\left(\psi_{\text{displ}}\left(\viewfull\right)\right) \in \mathbb{R}^{512}
\end{align}
% and likewise for $\Psi_{text{displ}}$ and $\viewdispl$. 
% The current estimate of the stylized mesh $\meshstyle$ is evaluated against the text prompt through rendering a 2D image $\view$ from viewpoint $\theta$. The CLIP embedding of the image $\view$ is obtained through a feed-forward pass of a pre-trained CLIP network $ {E}(\view) \in \mathbb{R}^{512}$. The target text prompt $t$ is similarly embedded through CLIP $ \phi_{text{target}} \in \mathbb{R}^{512}$.
% \rhc{we can say that CLIP removes the notion of spatial content... leaving behind an entangled notion of content and style in one vector.. } 
% The current estimate of the stylized mesh $\meshstyle$ is evaluated against the text prompt through rendering a 2D image. We leverage the differentiable renderer proposed by \cite{dibr}, to obtain a 2D image $I_{\theta}$ of the $\meshstyle$ taken from viewpoint $\theta$.
% pre-trained CLIP model to obtain a predicted style embedding $\hat{S}_i \in \mathbb{R}^{512}$. 
% Next, we embed the target image $I$ and text prompt $t$ using CLIP to obtain an embedding $\phi_{text{target}}$. We then normalize the $\hat{S}_i$'s and $\phi_{text{target}}$. Our loss is then given by: 
% Following the augmentations, we average the CLIP embeddings across all sampled views:
% \begin{align}
% \hat{S}^{\text{full}} = \frac{1}{n_{\theta}}\sum^{n_{\theta}}_{i=1}\hat{S}^{\text{full}}_{\theta_i} ~~~~~~~~~~~~~
% \hat{S}^{\text{displ}} = \frac{1}{n_{\theta}}\sum^{n_{\theta}}_{i=1}\hat{S}^{\text{displ}}_{\theta_i}
% \label{eq:viewavg}
% \end{align}
% That is, we regard the representation of the input mesh as the average of its embedding from multiple views.
The target $t$ is similarly embedded through CLIP by $\phi_{\text{target}} = E\left(t\right) \in \mathbb{R}^{512}$. 
% \begin{align}
% \phi_{\text{target}} = E\left(t\right) \in \mathbb{R}^{512}
% \end{align}
Our loss is then: % , $\mathcal{L}_{\text{sim}}$, is then: 
% \begin{align}
%      - \Bigl[ &\text{sim}\left(\hat{S}^{\text{full}}, \phi_{text{target}}\right) + \text{sim}\left(\hat{S}^{\text{displ}}, \phi_{text{target}}\right) \label{eq:fullloss}\\&+  \text{sim}\left(\hat{S}^{\text{local}}, \phi_{text{target}}\right) \Bigr]  
%      \label{eq:displloss}
% \end{align}
\begin{align}
     &\mathcal{L}_{\text{sim}} = \sum_{\hat{S}}\text{sim}\left(\hat{S}, \phi_{\text{target}}\right)
     \label{eq:fullloss}
     % \label{eq:displloss}
\end{align}
where $\hat{S} \in \{\hat{S}^{\text{full}}, \hat{S}^{\text{displ}}, \hat{S}^{\text{local}}  \}$ and 
% the cosine similarity between the mean embedding and the encoded target embedding. Formally:
% \begin{align}
%     \mathcal{L}_{\text{sim}} &= -\text{sim}(\frac{1}{n_{\theta}}\sum^{n_{\theta}}_{i=1} \hat{S}^{\text{full}}_{\theta_i}, \phi_{text{target}})\\&- \text{sim}(\frac{1}{n_{\theta}}\sum^{n_{\theta}}_{i=1} \hat{S}^{\text{displ}}_{\theta_i}, \phi_{text{target}})
% \end{align}
% \sagie{are augmentations randomly sampled once? it looks like it now, if not we should use and expectation notation with sampling}
% \ojm{Correct loss I think. Can someone verify?}
% \begin{align}
% \label{eq:simiarity} \mathcal{L}_{\text{sim}} = &\sum^M_i - \text{sim}(\frac{1}{n_{\theta}}\sum^{n_{\theta}}_\theta \hat{S}^{\text{full}}_{\theta_1}, \phi_{text{target}})  \\
% & \label{eq:simiarity_b}
% - \sum^4_1 \text{sim}(\frac{1}{n_{\theta}}\sum^{n_{\theta}}_{\theta} \hat{S}^{\text{full}}_{\theta_2}, \phi_{text{target}}) \\
% & \label{eq:simiarity_c} - \sum^4_1 \text{sim}(\frac{1}{n_{\theta}}\sum^{n_{\theta}}_{\theta} \hat{S}^{\text{displ}}_{\theta_2}, \phi_{text{target}})  
% \end{align}
$\text{sim}\left(a, b\right) = \frac{a \cdot b}{\left|a\right|\cdot\left|b\right|}$ is the cosine similarity between $a$ and $b$. We repeat the above with new sampled augmentations $n_{\text{aug}}$ times for each iteration. We note that the terms using $\hat{S}^{\text{full}}$ and $\hat{S}^{\text{local}}$ 
% in \ref{eq:fullloss} 
update $N_s$, $N_c$ and $N_d$ while the term using $\hat{S}^{\text{displ}}$  only updates $N_s$ and $N_d$. The separation into a \textit{geometry-only} loss and \textit{geometry-and-color} loss is an effective tool for encouraging meaningful changes in geometry ($-displ$ in \cref{fig:ablations}).
% \rhc{, intuition about why we use the geometric loss (comment from greg),} 

\subsection{Viewpoints and Augmentations}
\label{sec:viewpoint}
Given an input 3D mesh and target text, we first find an \emph{anchor} view. We render the 3D mesh at uniform intervals around a sphere and obtain the CLIP similarity for each view and target text. We select the view with the highest (\ie best) CLIP similarity as the \textit{anchor} view. 
Often there are multiple high-scoring views around the object, and using any of them as the anchor will produce an effective and meaningful stylization. See Supplementary for details.

We render multiple views of the object from randomly sampled views using a Gaussian distribution centered around the anchor view (with SD of $\pi$/4). 
We average over the CLIP-embedded views prior to feeding them into our loss, which encourages the network to leverage view consistency. 
For all our experiments, $n_\theta=5$ (number of sampled views). We show in the supplementary that
%$n_\theta$ to $3$ or $4$ is just as effective, 
% e 
setting $n_\theta$ beyond $5$ does not meaningfully impact the results.

\begin{figure}
    \centering
    \newcommand{\pl}{28}
    \begin{overpic}[width=\columnwidth]{figures/viewconsistency.jpg}
    \put(35,  \pl){\textcolor{black}{\textit{Robot alien}}}
    \end{overpic}
    \vspace{-25pt}
    \caption{Our neural texture field stylizes the entire 3D shape. \rhc{rinon doesnt like that the back is weird}}
    % Input text prompt: `Goat made of brick'.}
    \label{fig:viewconsistency}
    \vspace{-0.3cm}
\end{figure}
% As shown in \cref{sec:priors}, generating augmentations through $\Psi_{text{full}}$ and $\Psi_{text{displ}}$ is critical for our method to avoid degenerate solutions while generating fine-grained local geometric details. In our setting, a degenerate solution occurs when the stylized mesh contains severe artifacts and noise, despite having a high CLIP similarity to the target.
% For example, \cref{fig:synergy} shows that styling just the vertex colors is able to produce a result with equivalent CLIP similarity to styling both geometry and color, despite the clear visual deficiency (flatness) in the color style. \rhc{todo: maybe we should use the no geometric prior as the example here?} \rl{I agree -- I think that's a better example since it emphasizes how CLIP was trained in 2D so can ignore geometry.}
% Furthermore, existing CLIP-based synthesis works also observe that the pre-trained CLIP embedding is full of degenerate examples~\cite{Fort2021CLIPadversarial, Fort2021CLIPadversarialstickers,clipdraw, patashnik2021styleclip}. 

The 2D augmentations generated using $\Psi_{\text{full}}$ and $\Psi_{\text{displ}}$ are critical for our method to avoid degenerate solutions (see \cref{sec:priors}). $\Psi_{\text{full}}$ involves a random perspective transformation and $\Psi_{\text{displ}}$ generates both a random perspective and a random crop that is 10\% of the original image. Cropping allows the network to focus on localized regions when making fine grained adjustments to the surface geometry and color. 
% \rl{We need that color line figure that explains the effect of the perspective augmentation} \sagie{possibly additional fig for using nc and nd seperately}
%The crucial role of the perspective augmentation is not immediately obvious. \rhc{wdyt? sagie?}
% We note that other works that leverage CLIP-based representations, such as \cite{clipdraw}, also experience a drastic decline in output quality without the perspective augmentation. 
% We hypothesize that the perspective augmentation serves a key regularizing role in \textit{jittering} the embedding of the predicted style sufficiently to push the network out of the many degenerate solutions present in CLIP space. \rl{We need that color line figure that explains the effect of the perspective augmentation} \sagie{just show an ablation here - just as we have without crop, lets do without perspective, then we dont need to hypothesize}.
% \roi{I think we should mention the fact that we apply augmentation different than the identity with probability $p<1$, to avoid leakage of the augmentation to our generated results, following \cite{Stylegan-Ada}} \sagie{let's mention this in the supplementary} 
% Furthermore, there is a fundamental connection between color and geometry when it comes to defining style. 
% As shown in \cref{sec:geometrycolor}, the updates to shading and local geometry complement each other in identifying the areas of a surface that can be textured with a regular structure while preserving the shape's semantic parts. \sagie{moving to experimental part}
% \sagie{last sentence is amiguous and unclear - what did you mean?} 
% By sharing both local and global information between $\ndisplacement$ and $\ncolor$, better results are achieved than training each style attribute (color or displacement) individually, as shown in \cref{fig:synergy}. \rhc{i dont think this shows that tho... we would need a seperate fig (which we can say we have in the supp if we wanna add one) that shows training a two non-branched networks together}
Additional details and are given in the supplementary. 

==> figures/ablations/05_experiments.tex <==
\section{Experiments}
We examine our method across a diverse set of input source meshes and target text prompts. We consider a variety of sources including: COSEG~\cite{coseg}, Thingi10K~\cite{Thingi10K}, Shapenet~\cite{chang2015shapenet}, Turbo Squid~\cite{turbosquid}, and ModelNet~\cite{modelnet}. Our method requires no particular quality constraints or preprocessing of inputs, and the breadth of shapes we stylize in this paper and the supplementary illustrates its ability to handle low-quality meshes in the wild. Meshes used in the main paper as well as in the supplementary contain an average of 79,366 faces, 16\% non-manifold edges, 0.2\% non-manifold vertices, and 12\% boundaries. Our method takes less than 25 minutes to train on a single GPU, and high quality results usually appear in less than 10 minutes. 

\rhc{low quality meshes.}

% \rhc{todo high level summary of experiments}
In \cref{sec:control}, we demonstrate the multiple control mechanisms enabled by our method.
% show the ability of our method to generate high quality stylizations with controls.
%%% baseline %%%
In \cref{sec:priors}, we conduct a series of ablations on the key priors in our method.  % that illustrate the unique role each plays in achieving our high quality stylizations. 
We further explore the synergy between learning color and geometry in tandem. 
% , which results in superior refinement to both attributes than when either is learned alone. 
We introduce a user study in \cref{sec:baseline} where our stylization is compared to the closest baseline.  
% , in which we ask participants to evaluate how effectively our stylization adheres to a target prompt. 
% We also compare against a baseline method in the same study. 
As far as we can ascertain, no existing approach can be fairly compared against our method. Thus, we build a baseline from an existing CLIP-guided image synthesis technique that uses a pre-trained VQGAN~\cite{vqganclipnotebook}. For each target text prompt, we fine-tune VQGAN to generate an image with high CLIP similarity to the target. This baseline is similar in spirit, but differs from our method since: (1) both content and style may change, and (2) it modifies an image which cannot be expected to achieve multi-view consistency. 
% As far as we can ascertain, the method most close to ours uses a pretrained VQ-GAN together with CLIP in order to manipulate an input source 2D image in a manner that semantically matches a target text prompt~\cite{vqganclipnotebook}. To compare to this baseline, we render the 3D mesh from the desired viewpoint resulting in a 2D input source image, and apply this baseline with this source rendered image and target text prompt. 
In \cref{sec:target}, we show that our method can easily generalize to other target modalities beyond text, such as images or 3D shapes. Finally, we discuss limitations in \cref{sec:limitations}. 

% We further demonstrate that our method can handle low-quality meshes in the wild;  We also show that our method can effectively style toward other targets such as an image, image + text, mesh and mesh + text.   \rhc{removed genus for now. 2 sounds small..Can we put something with a wicked high genus in the supp?} \sagie{need to add a summary of all we do}

\subsection{Neural Stylization and Controls}
\label{sec:control}
% \rhc{TODO: discuss the orientation, of corn / bricks, refer to a figure}
Our method generates details with high granularity while still maintaining global semantics and preserving the underlying content. For example in \cref{fig:gallery}, given a vase mesh and target text `colorful crochet', the stylized output includes knit patterns with different colors, while preserving the structure of the vase. In \cref{fig:humans}, our method demonstrates a global semantic understanding of humans. Different body parts such legs, head and muscles are stylized appropriately in accordance with their semantic role, and these styles are blended seamlessly across the surface to form a cohesive texture. Moreover, our neural style field generates structured textures which are aligned to sharp curves and features (see bricks in \cref{fig:teaser,fig:gallery} and supplementary).
% \rhc{not sure if this view stuff. belongs here:} 
We show in \cref{fig:viewconsistency} and in the supplementary our generated styles from multiple views. 
% Even though our method samples fewer views which are far away from the main center view. 

\noindent\textbf{Fine Grained Controls.}
Our network leverages a positional encoding where the range of frequencies can be directly controlled by the standard deviation $\sigma$ of the $\mathbf{B}$ matrix \cref{eq:positional}. 
% with direct control of the range of possible input frequency values to encode the input coordinates before passing them to the MLP. 
% As shown in \cref{eq:positional}, one can adjust the frequency vectors, so as to control the range of possible frequencies in the positional encoding. 
In \cref{fig:frequency}, we show the results of three different frequency values when stylizing a source mesh of a torus towards the target text `stained glass donut'. Increasing the frequency value increases the frequency of style details on the mesh and produces sharper and more frequent displacements along the normal direction.
\begin{figure}[h]
    \centering
    \newcommand{\pl}{-3.5}
    \begin{overpic}[width=\columnwidth]{figures/freqcontrolv2.jpg}
    \put(20,  \pl){\textcolor{black}{$\sigma = 3$}}
    \put(45,  \pl){\textcolor{black}{$\sigma = 5$}}
    \put(75,  \pl){\textcolor{black}{$\sigma = 8$}}
    \put(36,  27){\textcolor{black}{\textit{Stained glass donut}}}
    %  \put(5,  -3){\textcolor{black}{\rotatebox{90}{stained glass}}}
    \end{overpic}
    \caption{Increasing the range of input frequencies in the positional encoding using increasing SD $\sigma$ for matrix $\mathbf{B}$ in \cref{eq:positional}. }
    % increases the frequency of the synthesized texture. }
    \label{fig:frequency}
    \vspace{-0.3cm}
\end{figure}
We further demonstrate our method's ability to successfully synthesize styles of varying levels of specificity. \cref{fig:textspec} displays styles of increasing detail and specificity for two input shapes. Note the retention of the style details from each level of target granularity to the next. 
%  Our method correctly adapts to more fine grained textual style specifications, stylizing additional details. 
Though the primary mode of style control is through the text prompt, we explore the way the network adapts to the geometry of the source shape. In \cref{fig:geoprior}, the target text prompt is fixed to `cactus'. We consider different input source spheres with increasing protrusion frequency. Observe that both the frequency and structure of the generated style changes to align with the pre-existing structure of the input surface. This shows that our method has the ability to preserve the content of the input mesh without compromising the quality of the stylization. 
\begin{figure}
    \centering
    \newcommand{\pl}{-3}
    \small
    \begin{overpic}[width=\columnwidth]{figures/textprogression.jpg}
    \put(16,  \pl){\textcolor{black}{(a)}}
    \put(39,  \pl){\textcolor{black}{(b)}}
    \put(62,  \pl){\textcolor{black}{(c)}}
    \put(84,  \pl){\textcolor{black}{(d)}}
    %  \put(5,  -3){\textcolor{black}{\rotatebox{90}{stained glass}}}
    \end{overpic}
    \caption{Increasing the target text prompt granularity for a source mesh of a lamp and iron. Top row targets: (a). `Lamp', (b). `Luxo lamp', (c). `Blue steel luxo lamp', (d). `Blue steel luxo lamp with corrugated metal. Bottom row targets: (a). `Clothes iron', (b). `Clothes iron made of crochet', (c). `Golden clothes iron made of crochet', (d). `Shiny golden clothes iron made of crochet'.}
    \label{fig:textspec}
    \vspace{-0.3cm}
\end{figure}

Our ability to manipulate style over the same input mesh using a neural style field enables morphing capabilities (see \cref{fig:morph}).
Interpolation, or \textit{morphing}, between two meshes requires correspondence between the shapes. Since our stylization preserves the original mesh content, \ie adds color and a displacement along the normal direction, correspondence is known explicitly. To achieve morphing, we linearly interpolate between the style value (RGB and displacement) of every point on the mesh, for the two source meshes. \rhc{explai this better, and why its cool}   
\begin{figure}[h]
    \centering
    \newcommand{\pl}{-3}
    \begin{overpic}[width=\columnwidth]{figures/morph.jpg}
    % \put(1,  \pl){\textcolor{black}{Content}}
    % \put(2,  \pl){\textcolor{black}{target image}}
    % % \put(44,  \pl){\textcolor{black}{\textit{$-$aug}}}
    % \put(34,  \pl){\textcolor{black}{\textit{image}}}
    % \put(58,  \pl){\textcolor{black}{\textit{text}}}
    % \put(76,  \pl){\textcolor{black}{\textit{image \& text}}}
    \end{overpic} 
    % \vspace{-8pt}
    \caption{Interpolating between the geometry and color of two different stylizations (left: `ford mustang', right: `limousine').}
    % is possible since our neural style field preserves the original source mesh.}
    \label{fig:morph}
    \vspace{-0.3cm}
\end{figure}

% \rhc{Putting this in a comment because it feels like it should go somewhere else. we need text to describe the fact that our style field is a general function that is disentangled from the mesh triangulation, but we also need an experiment to show it. at least we can promise it in the supp. I feel this deserves it's own sub section. }

% \rhc{
% Our ability to manipulate style using a neural style field representation offers a number of unique advantages. First, as opposed to a UV-parameterization, our neural style field does not assume a specific input mesh resolution. \rhc{The neural field is general and can be queried at locations on the surface... show it...}
% Our implementation can handle meshes with up to $180$K triangles on a GPU with 11GB of VRAM\rhc{TODO update with specs}. We are able to render stylized objects using very high resolutions, as shown in the supplementary.  \rhc{also in the main paper? sagie?}
% }

\subsection{\ourmethod{} Priors}
\label{sec:priors}

Our method incorporates a number of priors that allow us to perform stylization without a pre-trained GAN. We show an ablation where each prior is removed in \cref{fig:ablations}. Removing the style field network (\textit{$-$net}), and instead directly optimizing the vertex colors and displacements, results in noisy and arbitrary displacements over the surface. In \cite{clipdraw} random 2D augmentations are necessary to generate meaningful CLIP-guided drawings. We observe the same phenomena in our method, whereby removing 2D augmentations results in a stylization completely unrelated to the target text prompt. Without Fourier feature encoding (\textit{$-$FFN}), the generated style loses all fine-grained details. %, as well as the ability to synthesize interesting\rhc{??}. 
With the cropping augmentation removed (\textit{$-$crop}), the output is similarly unable to synthesize the fine-grained style details that define the target. Removing the \textit{geometry-only} component of $L_{sim}$ (\textit{$-$displ}) hinders geometric refinement, and the network instead compensates by simulating geometry through shading (see also \cref{fig:synergy}).
Without a geometric prior (\textit{$-$3D}) there is no source mesh to impose global structure, thus, the 2D plane in 3-space is treated as an image canvas.
%\rl{SCORES. Full: 0.361, Network: 0.260, FFN: 0.264, Aug: 0.199, No crop: 0.298, 3D: 0.286}
 % on which style is produced. 
% In theory, while the network could synthesize a globally coherent 2D candle on the image plane to match the target prompt, we hypothesize this is extremely difficult to do without the pre-defined object structure provided by the mesh.  
% \rhc{comment on the fact that there is still some interesting geometric deformations, but there's no global structure / awareness imposed in the result}

For each result in \cref{fig:ablations}, we report the CLIP similarity score, $\text{sim}(\hat{S}^{\text{full}}, \phi_{target})$, as defined in Sec.~\ref{sec:method}.
Our method obtains the highest score across different ablations, see \cref{fig:ablations}. 
% CLIP scores (ideally) reflect the significance of each of our priors. We do observe a correlation between visual quality and CLIP scores.
Ideally, there is a correlation between visual quality and CLIP scores.
% , which would reflect the significance of each of our priors.
However, \textit{-3D} manages to achieve a high CLIP similarity, despite its zero regard for global content semantics. This shows an example of how CLIP may naively prefer degenerate solutions, while our geometric prior steers our method away from these solutions.

% The scores are\rhc{TODO TODO TODO why are these numbers different from the figure caption?!?} $0.36$, $0.26$, $0.20$, $0.26$, $0.30$, $0.29$, and $0.29$ for the full, \textit{-net},\textit{-aug}, \textit{-FFN}, \textit{-crop}, \textit{-displ} and \textit{-3D} methods, respectively. 
% As seen in \cref{fig:ablations}, our method obtains the highest score across different ablations.
% indicating a correlation between visual quality and CLIP similarity. 
% However \textit{-3D} still manages to achieve a relatively high CLIP similarity score despite showing no awareness for global content semantics. The fact that CLIP contains degenerate solutions necessitates our method's effective use of priors in avoiding these solutions.\ojm{TODO: rana}
% % \sagie{user study here?}
% \rhc{Talk about some of the adversarial stuff here... the fact that no 3D is so high, yet looks globally unaware actually demonstrates the exact pitfalls of clip...}
\begin{figure}[h]
    \centering
    \newcommand{\pl}{-4}
    \begin{overpic}[width=\columnwidth]{figures/geometricprior.jpg}
    % \put(45,  40){\textcolor{black}{\textit{Cactus}}}
    \end{overpic}
    \caption{Texturing input source spheres (yellow) with protrusions of increasing frequency and with a fixed target of a `Cactus'. As can be seen, the final style frequency increases accordingly.}
    \label{fig:geoprior}
    \vspace{-0.4cm}
\end{figure}
% The geometric prior helps guide the structure of the style. When texturing spheres with protrusions of increasing frequency with the same target, the final style frequency increases as well. 
% \rhc{TODO: color inset of content with some color around the border and same with inset on the content. inset for middle one looks like it's a different scale.} \sagie{make it clear which inset is of the input mesh and which for the output}}

\noindent\textbf{Interplay of Geometry and Color.}\quad 
Our method utilizes the interplay between geometry and color for effective stylization, as shown in \cref{fig:synergy}. Learning to predict only geometric manipulations produces inferior geometry compared to learning geometry and color together, as the network attempts to simulate shading by generating displacements for self shadowing. An extreme case of this can be seen with the ``Batman" in \cref{fig:humans}, where the bat symbol on the chest is the result of a deep concavity formed through displacements alone. Similarly learning to predict only color results in the network attempting to hallucinate geometric detail through shading, leading to a flat and unrealistic texture that nonetheless is capable of achieving a relatively high CLIP score when projected to 2D. \cref{fig:synergy} illustrates this adversarial solution, where the ``Color" mode achieves a similar CLIP score as our ``Full" method.  
\begin{figure}[h]
    \centering
    \newcommand{\pl}{-3}
    \newcommand{\vl}{-8}
    \begin{overpic}[width=\columnwidth]{figures/geocolor_interplay.jpg}
    \put(35,  50){\textcolor{black}{\textit{Alien made of bark}}}
    \put(26,  \pl){\textcolor{black}{Full}}
    \put(50,  \pl){\textcolor{black}{Geometry}}
    \put(81,  \pl){\textcolor{black}{Color}}
    %
    \put(25,  \vl){\clipcolor{$0.322$}}
    \put(52,  \vl){\clipcolor{$0.250$}}
    \put(81,  \vl){\clipcolor{$0.320$}}
    \end{overpic}
    \vspace{1pt}
    \caption{Interplay between geometry and color for stylization. 
    % Our method exploits the interplay between geometry and color for stylization. 
    \textit{Full} - our method, \textit{Color} - only color changes, and \textit{Geometry} - only geometric changes. We also display the {\clipcolor{CLIP similarity}}. }
    % Modifying only geometry or color produces inferior geometry and flat color. \textit{Full} produces the highest {\clipcolor{CLIP similarity}} to the desired target text. \textit{Color} is able to hallucinate geometry which may deceptively increase CLIP similarlty scores}
    \label{fig:synergy}
    \vspace{-0.3cm}
\end{figure}


%%%% user study section %%%
\subsection{Stylization Fidelity}
\label{sec:baseline}
We conduct a user study to evaluate the perceived quality of the generated outputs, the degree to which they preserve the source content, and how well they match the target style. Since there is no technique which can fairly be compared against, we created a baseline using VQGAN-CLIP~\cite{vqganclipnotebook}. The VQGAN baseline synthesizes color inside the binary 2D mask projected from the 3D source shape (without 3D deformations) guided by CLIP. %
\rhc{emphasize why this is the right baseline. it works on general shapes, SMPL dude only only works on SMPL.}
% VQGAN receives an implicit content signal from the mask and an explicit one from the text prompt to generate a view of the stylized shape. 
% By incorporating a number of priors, we avoid the need to operate in a pretrained GAN latent space, as is the case in~\cite{patashnik2021styleclip, vqganclipnotebook}. Instead, we leverage CLIP's semantic and expressive embedding space to drive stylization.
\begin{table}
\newcommand{\allcolor}{\color[rgb]{0.4,0.4,0.95}}
\centering
\begin{tabular}{lccc} \\ 
\toprule
& (Q1): Overall & (Q2): Content & (Q3): Style  \\
\toprule
VQGAN & 2.83 &  3.60 & 2.59 \\
Ours & \textbf{3.90} &  \textbf{4.04} & \textbf{3.91} \\
\bottomrule
\end{tabular}
    \caption{User study. Mean opinion scores (range 1-5) for Q1-Q3 (see~\cref{sec:baseline}), for our method and baseline (control score: 1.16).
    }
\label{tab:user}
\vspace{-0.3cm}
\end{table}
We had 57 users evaluate $8$ random source meshes and style text prompt combinations. For each combination, we display the target text and the stylized output in pairs. The users are then asked to assign a score (1-5) to three factors: (Q1) ``How natural is the output depiction of \{\textit{content}\} + \{\textit{style}\}?" (Q2) ``How well does the output match the original \{\textit{content}\}?" (Q3) ``How well does the output match the target \{\textit{style}\}?" We report the mean opinion scores for each factor averaged across all style outputs for our method and the baseline in \cref{tab:user}. We also report a control score, which is the average score for 3 control questions in the survey where the target and outputs are deliberately mispaired. As expected, this score is close to 1. 
% We also report a control score based on quality control questions we ask where there is no relationship between the image and target text. These questions are used to filter out low quality respondents who might have either misunderstood the nature of the task or did not take the evaluation seriously. 
Our method outperforms the VQGAN baseline across all questions, with a difference of $1.07$, $0.44$, and $1.32$ for Q1-Q3, respectively. Though VQGAN is somewhat effective at representing the natural content in our prompts, perhaps due to the implicit content signal it receives from the mask, it struggles to synthesize these representations with style in a meaningful way. 
% VQGAN's higher performance on Q2 may be a result of the mask we pass it, which introduces an additional content signal beyond that supplied in the text prompt.
Visual examples of our method and the baseline are shown in the supplementary. Screenshots of our user study are also shown in the supplementary.

% \rhc{TODO: sagie....}
% \textbf{Making style symmetric}
% We leverage the neural priors again by introducing kernels that matches our problem-specific knowledge. That is using the the basic kernel tricks which are popular in improving classification solutions we can encourage symmetry in arbitrary axes and coordinate systems; periodical solutions \etc. Given a kernel function, the smoothness of the network would assign similar colors and displacements to points that are close in the kernel space.  \roi{TODO: people + ball} The fact that most meshes available online are not $100\%$ symmetric allows the network some degree of freedom - set different coloring on vertices that are very close under the kernel but requires different colors. This yields great results in practice.\ojm{This section should be rewritten by whoever did these experiments. The use of kernel is not correct here and what we are doing is much simpler, just mapping the left side to the right to get symmetry}


\label{sec:modality}
\begin{figure}[h]
    \centering
    \newcommand{\pl}{-3}
    \newcommand{\targetcolor}{\color[rgb]{0.1,0.33,0.57}}
    \begin{overpic}[width=\columnwidth]{figures/imagetarget.jpg}
    % \put(1,  \pl){\textcolor{black}{Content}}
    % \put(2,  \pl){\textcolor{black}{target image}}
    % % \put(44,  \pl){\textcolor{black}{\textit{$-$aug}}}
    % \put(34,  \pl){\textcolor{black}{\textit{image}}}
    % \put(58,  \pl){\textcolor{black}{\textit{text}}}
    % \put(76,  \pl){\textcolor{black}{\textit{image \& text}}}
    \end{overpic} 
    % \vspace{-8pt}
    \caption{Stylization driven by an {\targetcolor image target}. Our method can stylize meshes using an image to describe the desired style.}
    \label{fig:target}
    \vspace{-0.3cm}
\end{figure}
% \sagie{a more central role for this section?}
% While our framework tackles the novel application of stylization a source mesh using a target text prompt, it is in fact much more general, 
\subsection{Beyond Textual Stylization}
\label{sec:target}
Beyond text-based stylization, our method can be used to stylize a mesh toward different target modalities such as a 2D image or even a 3D object. For a target 2D image $I_t$, $\phi_{target}$ in \cref{eq:fullloss}, represents the image-based CLIP embedding of $I_t$. For a target mesh $T$, $\phi_{target}$ is the average embedding, in CLIP space, of the 2D renderings of $T$, where the views are the same as those sampled for the source mesh. 
% \ojm{TODO: need to write about target mesh (previous explanation was not correct)}\rhc{good that we explain this here, but I am not sure I remember the notation, can we also add the words of what this is?} \rl{We don't sample new views on the target, but rather take the same views the we sample for the source right?} 
Beyond different modalities, we can combine targets across different modalities by simply summing $\mathcal{L}_{sim}$ over each target. In Fig.~\ref{fig:target} we consider a source mesh of a pig with different image targets. In Fig.~\ref{fig:mesh2mesh}(a), we consider stylization using a target mesh and in Fig.~\ref{fig:mesh2mesh}(b), we combine both a mesh and text target to achieve the output style. Our method successfully adheres to the target style. 

\begin{figure}
    \centering
    \vspace{-5pt}
    \newcommand{\pl}{-2}
    \begin{overpic}[width=\columnwidth]{figures/m2m.png}
    \put(10,  \pl){\textcolor{black}{(a)}}
    \put(30,  \pl){\textcolor{black}{(b)}}
    \put(40,  \pl){\textcolor{black}{Target 1}}
    \put(60,  \pl){\textcolor{black}{(c)}}
    \put(75,  \pl){\textcolor{black}{(d)}}
    \put(88,  \pl){\textcolor{black}{Target 2}}
    \end{overpic}
    \caption{Neural stylization driven by mesh targets. (a-c) are styled using Targets 1 and 2. (b-c) are styled with text in addition to the mesh targets: (c) `a cactus that looks like a cow', (d) `a mouse that looks like a duck'. }
    \label{fig:mesh2mesh}
    \vspace{-0.3cm}
\end{figure}


%https://drive.google.com/drive/folders/1jGqb0lRkN8PjE2JDf1C538xT9wi-Sfp7?usp=sharing
\subsection{Limitations}
\label{sec:limitations}
Our method implicitly assumes there exists a synergy between the input 3D geometry and the target style prompt (see \cref{fig:limitations}). However, stylizing a 3D mesh (\eg, dragon) towards an unrelated/unnatural prompt (\eg, \textit{stained glass}) may result in a stylization that ignores the geometric prior and effectively erases the source shape content. Therefore, in order to preserve the original content when editing towards a mismatched target prompt, we simply include the object category in the text prompt (\eg, \textit{stained glass dragon}), thus semantically embedding a content preservation constraint directly into the target. 
% In addition, we find that sometimes unwanted artifacts can appear at random throughout the mesh. Interestingly, these artifacts usually take the form of a face or facial features such as eyes or a mouth. Examples of such artifacts can be found in Figures \ref{fig:teaser}, \ref{fig:gallery},\ref{fig:viewconsistency} ,\ref{fig:synergy} and \ref{fig:mesh2mesh}. We suspect that because a significant amount of CLIP's training data may contain faces, and these artifacts give the network an easy way to increase the CLIP similarity of its generated output. We also observe geometric artifacts, where objects may appear shriveled up or overly stretched due to improper scaling along their normal direction.\ojm{Should we also include a figure of just plain bad results?}
% Our method does not make any assumptions on the quality of the input mesh, but does assume that the user knows the shape semantic category and sets a reasonable center view point for sampling around. W
%
% With regards to the choice of anchor view (\ref{sec:method}), we observe in practice that our method is robust to many choices of the anchor view, though as shown in the supplementary, certain views that are distant from key semantic features of the shape, e.g. the bottom view of the goat, result in a poor or incomplete stylization.
% \rhc{ideas to mention: we assume that we know the object category.} 
% \sagie{TALK ABOUT LIMITATIONS FIGURE AND ALSO OTHER LIMITATIONS}
\begin{figure}
    \centering
    \newcommand{\pl}{-3}
    \newcommand{\tl}{1}
    \begin{overpic}[width=\columnwidth]{figures/limitations_fig.png}
        \put(5,  \pl){\textcolor{black}{Stained glass}}
        \put(35,  \tl){\textcolor{black}{Stained glass}}
        \put(39,  \pl){\textcolor{black}{{dragon}}}
        \put(63,  \pl){\textcolor{black}{Candy}}
        \put(82,  \tl){\textcolor{black}{Candy}}
        \put(80,  \pl){\textcolor{black}{aramdillo}}
    \end{overpic} 
    % \vspace{-8pt}
    \caption{Geometric content and target style synergy. If the target style is unrelated to the 3D mesh content, the stylization may appear to ignore the 3D content. Results are improved when including the content in the target text prompt.}
    \label{fig:limitations}
    \vspace{-0.3cm}
\end{figure}

% \rhc{
% \begin{figure}
%     \centering
%     \newcommand{\pl}{95}
%     \newcommand{\tl}{1}
%     \begin{overpic}[width=\columnwidth]{figures/sampleviews.jpg}
%         \put(45,  \pl){\textcolor{black}{\textit{Goat in a poncho}}}
%     \end{overpic} 
%     % \vspace{-8pt}
%     \caption{A poor choice of center view may result in a failure to achieve a global and view-consistent texturing. Center views are shown in black outline on the left, with other views of the resulting texture for each row on the right.}
%     \label{fig:viewlimitations}
% \end{figure}
% }

==> figures/ablations/06_conclusion.tex <==
\section{Conclusion}

% \sagie{NEEDS TO BE SHORTNED}

We presented a novel framework for \emph{stylizing} input meshes given a target text prompt. Our framework learns to predict colors and local geometric details using a neural stylization field. It can predict structured textures (\eg bricks), without a directional field or mesh parameterization. Traditionally, the direction of texture patterns over 3D surfaces has been guided by 3D shape analysis techniques (as in \cite{xu2009feature}). In this work, the texture direction is driven by 2D rendered images, which capture the semantics of how textures appear in the real world.

% Multiple 2D renderings of edited 3D content generates a strong signal to guide neural stylization.
% , despite never training on 3D content explicitly.
Without relying on a pre-trained GAN network or a 3D dataset, we are able to manipulate a myriad of meshes to adhere to a wide variety of styles. Our system is capable of generating out-of-domain stylized outputs, \eg, a stained glass shoe or a cactus vase (\cref{fig:gallery}). 
%
Our framework uses a pre-trained CLIP~\cite{clip} model, which has been shown to contain bias~\cite{agarwal2021evaluating}. We postulate that our proposed method can be used to visualize, understand, and interpret such model biases in a more direct and transparent way.
%(extended discussion in the supplementary material). 
% Our method implicitly assumes there exists a synergy between the input 3D geometry and the desired style (see \cref{fig:limitations}). However, stylizing a 3D mesh (\eg, dragon) towards an unrelated text prompt (\eg, \textit{stained glass}) may result in a stylization that ignores the geometric prior, \ie, 3D content \emph{erasing}. Therefore, in order to preserve the original content when editing towards mismatched target prompt, we simply incorporate the object category in the text prompt (\eg, \textit{stained glass dragon}).

% \begin{figure}[h]
%     \centering
%     \newcommand{\pl}{-3}
%     \newcommand{\tl}{1}
%     \begin{overpic}[width=\columnwidth]{figures/limitations_fig.png}
%         \put(5,  \pl){\textcolor{black}{Stained glass}}
%         \put(35,  \tl){\textcolor{black}{Stained glass}}
%         \put(39,  \pl){\textcolor{black}{{dragon}}}
%         \put(63,  \pl){\textcolor{black}{Candy}}
%         \put(82,  \tl){\textcolor{black}{Candy}}
%         \put(80,  \pl){\textcolor{black}{aramdillo}}
%     \end{overpic} 
%     % \vspace{-8pt}
%     \caption{Geometric content and target style synergy. If the target style is unrelated to the 3D mesh content, the stylization may appear to ignore the 3D content. Results are improved when including the content in the target text prompt.}
%     \label{fig:limitations}
% \end{figure}
% Our method implicitly assumes there exists a synergy between the input 3D geometry and the desired style (see \cref{fig:limitations}). However, stylizing a 3D mesh (\eg, dragon) towards an unrelated text prompt (\eg, \textit{stained glass}) may result in a stylization that ignores the geometric prior, \ie, 3D content \emph{erasing}. Therefore, in order to preserve the original content when editing towards mismatched target prompt, we simply incorporate the object category in the text prompt (\eg, \textit{stained glass dragon}).
% synthesizing truly unrelated styles onto a 3D mesh  may trivially result in content

% We have achieved this by specifying the object category in the text prompt. \rhc{Since the latent CLIP embedding actually does entangle content and style, we should }


% This work takes a first step towards synthesis possibilities with 3D content. 
% In this work we presented a technique for manipulating the \emph{style} of 3D meshes,
As future work, our framework could be used to manipulate 3D \emph{content} as well. 
%The content of an object could be modified through smooth and low-frequency deformations, in order to modify the object's pose or non-local structure~\cite{neuralcages, li2021learning}. 
Instead of modifying a given input mesh, one could learn to synthesize meshes from scratch driven by a text prompt.
% We are particularly keen on an approach which could generate 3D meshes with varying genus. 
Moreover, our neural style field is tailored to a single 3D mesh. It may be possible to train a network to stylize a collection of meshes towards a target style in a feed-forward manner. 
% Leveraging a small dataset or training the neural style network to be conditioned on different styles as input over a single shape.


==> figures/vqgan/table.tex <==
\begin{table*}
\adjustimage{width=5cm,valign=c}{figures/vqgan/vases-user.png}\quad%
\begin{tabular}{l c c | c c | c c | c c | c c} % centered columns (4 columns)
\hline
& \multicolumn{2}{c}{\textbf{Anchor}} & \multicolumn{2}{c}{\textbf{Daratech}}  & \multicolumn{2}{c}{\textbf{DC}} & \multicolumn{2}{c}{\textbf{Gargoyle}} & \multicolumn{2}{c}{\textbf{Lord Quas}} \\
\hline\hline %inserts double horizontal lines
\textbf{Method} & score & faces & score & faces & score & faces & score & faces & score & faces\\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
APSS & 97.1 & 347K & 96.4 & 196K & 98.4 & 302K & 98.5 & 363K & 99.5 & 175K \\ 
DGP & 95.9 & 4M & 95.2 & 4M & 96.5 & 4M & 96.0 & 4M & 97.7 & 4M \\ 
EAR & 96.3 & NA & 95.4 & NA & 96.5 & NA & 97.4 & NA & 98.0 & NA \\ 
Fourier & 94.9 & NA & 93.3 & NA & 98.5 & NA & 98.4 & NA & 98.6 & NA \\ 
IMLS & 96.9 & 358K & 96.3 & 205K & 98.4 & 309K & 97.9 & 262K & 99.2 & 178K \\ 
MPU & 97.5 & 240K & 95.6 & 94K & 99.0 & 210K & 98.5 & 162K & 98.9 & 104K \\ 
MPUS & 97.6 & 224K & 95.0 & 90K & 99.3 & 207K & 99.1 & 267K & 99.0 & 103K \\ 
Poisson & 94.2 & 552K & 97.6 & 446K & 97.8 & 535K & 97.6 & 671K & 98.0 & 419K \\ 
SPoisson & 96.0 & 333K & 94.6 & 269K & 99.0 & 322K & 98.9 & 404K & 99.5 & 253K \\ 
RBF & 95.5 & 246K & 92.2 & 149K & 99.1 & 236K & 90.2 & 289K & 99.3 & 168K \\ 
Spss & 92.8 & 351K & 92.2 & 208K & 97.4 & 302K & 97.5 & 258K & 98.9 & 174K \\ 
Wavelet & 94.4 & 158K & 86.3 & 145K & 95.9 & 195K & 97.4 & 162K & 97.5 & 150K \\ 
Ours & 96.7 & 14K & 96.9 & 15K & 98.9 & 40K & 98.8 & 34K & 98.9 & 10K \\ \\ [1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
\caption{Resultsof on surface reconstruction benchmark~\cite{berger2013benchmark} }
\label{table:sig13}
\end{table*}



%%

\begin{table}
\adjustimage{width=2cm,valign=c}{figures/vqgan/vases-user.png}\quad%
\begin{tabular}{l c c } % centered columns (4 columns)
\hline
& \multicolumn{2}{c}{\textbf{Mean Opinion Score}} \\
\hline\hline %inserts double horizontal lines
\textbf{Method} & score & faces \\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
APSS & X & X \\ 
Ours & X & X \\ %\\ [1ex] % [1ex] adds vertical space
% \hline %inserts single line
\end{tabular}
\caption{Caption.}
\label{table:sig13}
\end{table}


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
%     \centering
%     % element 1
%     \begin{tabular}{c|c|c|c}
%     % \hline
%     \multicolumn{4}{c}{\textbf{Mean Opinion Score}} \\
%     \hline
%      & overall &  content & style \\
%      \hline
%      VQGAN & X &  X & X \\
%      Ours & X &  X & X \\
%     \end{tabular}
%     % element 2
%     &
%     \includegraphics[height=2cm]{figures/vqgan/vases-user.png}
%     \\
%     \end{tabular}
%     \caption{User study. We polled \rhc{X} users on three aspects of the results; \emph{overall}: how natural the result depicts content \& style, how effective }
%     \label{tab:user}
% \end{table}


%%

\begin{table}[h]
    \adjustimage{width=2cm,valign=c}{figures/vqgan/vases-user.png}\quad%
    \begin{tabular}{cl}
    \centering
    % element 1
    \begin{tabular}{c|c|c|c}
    % \hline
    \multicolumn{4}{c}{\textbf{Mean Opinion Score}} \\
    \hline
     & overall &  content & style \\
     \hline
     VQGAN & X &  X & X \\
     Ours & X &  X & X \\
    \end{tabular}
    % element 2
    &
    % \adjustbox{valign=T}{\includegraphics[height=1.5cm]{figures/vqgan/vases-user.png}}
    % \raisebox{-\totalheight}{\includegraphics[height=2cm]{figures/vqgan/vases-user.png}}
    \\
    \end{tabular}
    \caption{User study. We polled \rhc{X} users on three aspects of the results; \emph{overall}: how natural the result depicts content \& style, how effective }
    \label{tab:user}
\end{table}
